Propagation of chaos and large deviations in mean-field models with jumps on block-structured networks

A system of interacting multiclass finite-state jump processes is analyzed. The model under consideration consists of a block-structured network with dynamically changing multi-colors nodes. The interaction is local and described through local empirical measures. Two levels of heterogeneity are considered: between and within the blocks where the nodes are labeled into two types. The central nodes are those connected only to the nodes of the same block whereas the peripheral nodes are connected to both the nodes of the same block and to some nodes from other blocks. The limits of such systems as the number of particles tends to infinity are investigated. Under regularity conditions on the peripheral nodes, propagation of chaos and law of large numbers are established in a multi-population setting. In particular, it is shown that, as the number of nodes goes to infinity, the behavior of the different classes of nodes can be represented by the solution of a McKean-Vlasov system. Moreover, we prove large deviation principles for the vectors of empirical measures and the empirical processes.

==> babelbst.tex <==
%%
%% This is file `merlin.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% merlin.mbs  (with options: `bblbst')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from merlin.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file merlin.mbs.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
%% Copyright 1994-1999 Patrick W Daly
 % ===============================================================
 % IMPORTANT NOTICE:
 % This bibliographic style (bst) file has been generated from one or
 % more master bibliographic style (mbs) files, listed above.
 %
 % This generated file can be redistributed and/or modified under the terms
 % of the LaTeX Project Public License Distributed from CTAN
 % archives in directory macros/latex/base/lppl.txt; either
 % version 1 of the License, or any later version.
 % ===============================================================
 % Name and version information of the main mbs file:
 % \ProvidesFile{merlin.mbs}[1999/05/28 3.89 (PWD)]
 % This is babelbst.tex for English.
 % It should serve as a model for other languages.
 % Alternatively, store it under a different name (e.g. englbst.tex)
 % and then \input it with a command in babelbst.tex.
%\ifcase\language \input{frenbst} \or \input{frenbst}
%\else \input{frenbst} \fi
\def\bbland{et}                \def\bbletal{et~al.}
\def\bbleditors{r\'edacteurs}        \def\bbleds{r\'ed.}
\def\bbleditor{r\'edacteur}          \def\bbled{r\'ed.}
\def\bbledby{edit\'e par}
\def\bbledition{edition}        \def\bbledn{ed}
\def\bblvolume{tome}          \def\bblvol{vol.}
\def\bblof{de}
\def\bblnumber{num\'ero}          \def\bblno{n$^\mathrm{o}$}
\def\bblin{dans}
\def\bblpages{pages}            \def\bblpp{pp.}
\def\bblpage{page}              \def\bblp{p.}
\def\bblchapter{chapitre}        \def\bblchap{chap.}
\def\bbltechreport{Rapport technique}
\def\bbltechrep{Rap. Tech.}
\def\bblmthesis{Th\`ese de ma\^itre}
\def\bblphdthesis{Th\`ese de doctorat}
\def\bblfirst{Premi\`ere}            \def\bblfirsto{1ere}
\def\bblsecond{Deuxi\`eme}          \def\bblsecondo{2\`eme}
\def\bblthird{Troisi\`eme}            \def\bblthirdo{3\`eme}
\def\bblfourth{Quatri\`eme}          \def\bblfourtho{4\`eme}
\def\bblfifth{Cinqui\`eme}            \def\bblfiftho{5\`eme}
\def\bblst{$^{\mbox{\scriptsize \`ere}}$}  
\def\bblnd{$^{\mbox{\scriptsize \`eme}}$}  
\def\bblrd{$^{\mbox{\scriptsize \`eme}}$}
\def\bblth{$^{\mbox{\scriptsize \`eme}}$}
\def\bbljan{janvier}  \def\bblfeb{f\'evrier}  \def\bblmar{mars}
\def\bblapr{avril}    \def\bblmay{mai}       \def\bbljun{juin}
\def\bbljul{juillet}     \def\bblaug{ao\^ut}    \def\bblsep{septembre}
\def\bbloct{octobre}  \def\bblnov{novembre}  \def\bbldec{d\'ecembre}
\endinput
%%
%% End of file `merlin.tex'.

